Robust and Verifiable Information Embedding Attacks to Deep Neural Networks via Error-Correcting Codes

In the era of deep learning, a user often leverages a third-party machine learning tool to train a deep neural network (DNN) classifier and then deploys the classifier as an end-user software product or a cloud service. In an information embedding attack, an attacker is the provider of a malicious third-party machine learning tool. The attacker embeds a message into the DNN classifier during training and recovers the message via querying the API of the black-box classifier after the user deploys it. Information embedding attacks have attracted growing attention because of various applications such as watermarking DNN classifiers and compromising user privacy. State-of-the-art information embedding attacks have two key limitations: 1) they cannot verify the correctness of the recovered message, and 2) they are not robust against post-processing of the classifier. In this work, we aim to design information embedding attacks that are verifiable and robust against popular post-processing methods. Specifically, we leverage Cyclic Redundancy Check to verify the correctness of the recovered message. Moreover, to be robust against post-processing, we leverage Turbo codes, a type of error-correcting codes, to encode the message before embedding it to the DNN classifier. We propose to recover the message via adaptively querying the classifier to save queries. Our adaptive recovery strategy leverages the property of Turbo codes that supports error correcting with a partial code. We evaluate our information embedding attacks using simulated messages and apply them to three applications, where messages have semantic interpretations. We consider 8 popular methods to post-process the classifier. Our results show that our attacks can accurately and verifiably recover the messages in all considered scenarios, while state-of-the-art attacks cannot accurately recover the messages in many scenarios.

==> discussion.tex <==
\section{Discussion and Limitations}
\label{discussion}

\myparatight{Classifier's accuracy} Both existing and our new information embedding attacks slightly sacrifice the accuracy of the learnt classifier. Moreover, our information embedding attacks sacrifice slightly more accuracy than existing attacks, because our attacks embed larger messages to the classifier due to error-correcting codes.   However, the accuracy losses are within 1\%, which are acceptable. Moreover, the user may not notice such small difference, i.e., the user may not be able to tell whether a classifier produced by a machine learning tool has embedded messages or not via examining the classifier's accuracy. 


\myparatight{Number of queries} Compared to existing information embedding attacks~\cite{song2017machine}, our attacks are verifiable and robust against multiple post-processing methods because our attacks leverage error-detecting and error-correcting codes. For the same reason, our attacks require comparable or several times more queries than existing attacks. We stress that requiring several times more queries is acceptable in practice. Specifically, when the classifier is deployed as an end-user software, attacker can send an arbitrary number of queries to the classifier once the attacker obtains the software. When the classifier is deployed as a cloud service, the cloud service may charge customers based on the number of queries. Therefore, our attacks may incur several times more economic cost for attacker. However, the cost per query is very small, e.g., \$$5\times 10^{-4}$ per query on IBM Watson Machine Learning~\cite{IBM}. As a result, the total economic cost for the attacker is still small. 



\myparatight{Using confidence scores and model parameters to embed the message} In this work, we consider the message is represented using the labels of some data points, which is generally applicable even if the attacker does not have access to the confidence scores predicted by the classifier or the model parameters of the classifier. However, if the classifier's prediction API also outputs confidence scores for a query, then the attacker could leverage them to embed and recover the message. Moreover, if the attacker has access to the classifier's model parameters, e.g., via reverse engineering the end-user software product, the attacker could also embed the message into the model parameters. It is an interesting future work to explore verifiable and robust information embedding in such scenarios. 


\myparatight{Relationship and difference with watermarking} Watermarking multimedia data such as images has been extensively studied~\cite{hartung1999multimedia}. For example, a watermark can be embedded into an image without sacrificing the image quality and later recovered. Error-correcting codes were also applied to make multimedia watermarking more robust~\cite{baudry2001analyses}. Watermarking techniques were recently extended to protect the intellectual property of deep neural networks. Specifically, a model owner can embed a watermark to its model during training. Suppose some entity pirated the model and deploys it as a software or cloud service, which we call \emph{deployed model}. The model owner can check whether the {deployed model} is a pirated version of its model using watermarking.  In particular, if the model owner can recover its watermark from the deployed model, then the deployed model may belong to the model owner. The watermarking techniques for neural networks are different from those for multimedia data because neural networks have their own special characteristics. % and requirements. 
For instance,  the watermark should be embedded in  a way that does not significantly sacrifice the neural network's accuracy. 

Existing watermarking techniques for neural networks can be classified into two categories, i.e., \emph{white-box watermarking}~\cite{uchida2017embedding,rouhani2018deepsigns} and \emph{black-box watermarking}~\cite{zhang2018protecting,adi2018turning}. In  white-box watermarking, the watermark is embedded into the parameters of the model owner's model, while the watermark is embedded into the labels of some data points in  black-box watermarking.   White-box watermarking requires access to the parameters of the deployed model in order to recover the watermark, while black-box watermarking only requires access to the deployed model's prediction API. In particular, existing black-box watermarking methods~\cite{zhang2018protecting,adi2018turning} essentially select an attack dataset as watermark and only use Step IV of our information embedding attacks to embed the watermark into the model owner's neural network model. For a deployed model, the model owner queries its API to predict the labels of the data points in the attack dataset. If the labels predicted by the deployed model match those predicted by the model owner's model, then the model owner predicts that the deployed model is a pirated version of its model. 

Our information embedding attacks can be used for black-box watermarking. Specifically, a model owner could select an (arbitrary) message as a watermark and embed the message into its neural network during training using our Embed function. For a deployed model, the model owner can use our Recover function to recover the message/watermark via querying the deployed model's prediction API. If the recovered message is the same or similar to the message the model owner embeds into its own model, then the model owner predicts that the deployed model is a pirated version of its model. Comparing with existing black-box watermarking methods, our information embedding attacks based watermarking is more robust against post-processing, as we leverage error-correcting codes to introduce redundancy in the message/watermark.  It is an interesting future work to  apply error-correcting codes to white-box watermarking for neural networks. 




\myparatight{Detecting random queries} Our information embedding attacks require querying the labels of the data points in the attack dataset. Moreover, the data points in our attack dataset are randomly generated, whose distribution may be different from the training data distribution. Therefore, the user could detect our information embedding attacks via analyzing the statistics of the queries. Specifically, if the queries from the same customer follow a distribution that is significantly different from the training data distribution, the service (especially a cloud service) may block the customer. Such statistical method~\cite{Kesarwani18} was proposed to detect model parameter stealing attacks in Machine Learning as a Service.    However, the attacker could register multiple customers and distribute the queries among them, which could  evade such statistical detection methods. 

\myparatight{Model parameter stealing attacks} We showed that our information embedding attacks can be used to perform training data, property, and neural network architecture inference attacks. In principle, information embedding attacks could also be used to perform model parameter stealing attacks~\cite{tramer2016stealing}, i.e., we represent the model parameters as a message. However, we found that the message that represents model parameters is very large for neural networks. For instance, even if we compress  the model parameters of the ResNet model for the CIFAR10 dataset using rar, the compressed parameters are still around 1MB. Embedding such a large message into a neural network requires a large attack dataset, which impacts the classifier's accuracy significantly. 










